ee$\in$MC: Simulation of $\bf e^{+}e^{-} \to \mu^{+} \mu^{-} (\gamma) $ and $\bf e^{+}e^{-} \to \tau^{+}\tau^{-} (\gamma) $ Events

We present a new Monte-Carlo generator, {\tt ee$\in$MC}, for the simulation of $e^{+}e^{-} \to \mu^{+} \mu^{-} (\gamma) $, $e^{+}e^{-} \to \tau^{+}\tau^{-} (\gamma) $ and $\tau$ lepton decays which is suitable for $e^{+}e^{-}$ colliders from threshold up to energy of $\sim 10.58GeV$. The $e^{+}e^{-} \to \mu^{+} \mu^{-}(\gamma) $, $e^{+}e^{-} \to \tau^{+}\tau^{-}(\gamma)$ interactions are computed up to the exact LO matrix element where the running of $\alpha_{QED}$ includes both the LO leptonic and hadronic vacuum polarization. Infra-red divergences are investigated within the Yennie-Frautschi-Suura Exponentiation formalism, where several well-known approximations and a formulation based on the exact LO contribution to the soft and virtual photons are applied. The simulation of the $\tau$ lepton consists of the leptonic decay modes at Born level and theoretical models based on Flux-Tube Breaking Models and Chiral Resonance Lagrangian Models as well as experimental models for the majority of semi-leptonic decay modes. This includes hadronic models for investigating the origin of low mass scalar sector recently observed in decays of the $\tau$ lepton and their association with the origin of the constituent-quark mass through Chiral-symmetry Breaking.

==> ExponentiationTable.tex <==
\\ \hline 
\multicolumn{7}{c}{Exponentiation Type I} \\ 
 \hline 
$ 2.1 m_{\mu} $ & 790.8 & 850.3 & 789.5 & \multicolumn{1}{c}{$-$} & \multicolumn{1}{c}{$-$} & \multicolumn{1}{c}{$-$} \\ 
0.5 & 377.5 & 394.4 & 345.7 & \multicolumn{1}{c}{$-$} & \multicolumn{1}{c}{$-$} & \multicolumn{1}{c}{$-$} \\ 
1 & 95.80 & 98.09 & 88.06 & \multicolumn{1}{c}{$-$} & \multicolumn{1}{c}{$-$} & \multicolumn{1}{c}{$-$} \\ 
2 & 24.24 & 24.20 & 22.58 & \multicolumn{1}{c}{$-$} & \multicolumn{1}{c}{$-$} & \multicolumn{1}{c}{$-$} \\ 
$ 2.1 m_{\tau} $ & 6.982 & 6.792 & 6.685 & 3.261 & 3.522 & 6.661 \\ 
5 & 3.800 & 3.652 & 3.682 & 3.702 & 3.934 & 3.695 \\ 
10.58 & 0.8176 & 0.7602 & 0.8398 & 0.9503 & 0.9795 & 0.8373 \\ 
\hline 
\multicolumn{7}{c}{Exponentiation Type II} \\ 
 \hline 
$ 2.1 m_{\mu} $ & 799.3 & 859.4 & 789.5 & \multicolumn{1}{c}{$-$} & \multicolumn{1}{c}{$-$} & \multicolumn{1}{c}{$-$} \\ 
0.5 & 381.5 & 398.6 & 345.7 & \multicolumn{1}{c}{$-$} & \multicolumn{1}{c}{$-$} & \multicolumn{1}{c}{$-$} \\ 
1 & 96.83 & 99.14 & 88.06 & \multicolumn{1}{c}{$-$} & \multicolumn{1}{c}{$-$} & \multicolumn{1}{c}{$-$} \\ 
2 & 24.50 & 24.46 & 22.58 & \multicolumn{1}{c}{$-$} & \multicolumn{1}{c}{$-$} & \multicolumn{1}{c}{$-$} \\ 
$ 2.1 m_{\tau} $ & 7.057 & 6.865 & 6.685 & 3.296 & 3.560 & 6.661 \\ 
5 & 3.840 & 3.691 & 3.682 & 3.742 & 3.976 & 3.695 \\ 
10.58 & 0.8264 & 0.7683 & 0.8398 & 0.9605 & 0.9900 & 0.8373 \\ 
%10.58 & 0.82645 & 0.7685 & 0.8413 & 0.9608 & 0.9893 & 0.8414 \\
\hline 
\multicolumn{7}{c}{Exponentiation Type III} \\ 
 \hline  
$ 2.1 m_{\mu} $ & 785.3 & 839.8 & 789.5 & \multicolumn{1}{c}{$-$} & \multicolumn{1}{c}{$-$} & \multicolumn{1}{c}{$-$} \\ 
0.5 & 370.6 & 386.9 & 345.7 & \multicolumn{1}{c}{$-$} & \multicolumn{1}{c}{$-$} & \multicolumn{1}{c}{$-$} \\ 
1 & 92.68 & 95.16 & 88.06 & \multicolumn{1}{c}{$-$} & \multicolumn{1}{c}{$-$} & \multicolumn{1}{c}{$-$} \\ 
2 & 23.19 & 23.15 & 22.58 & \multicolumn{1}{c}{$-$} & \multicolumn{1}{c}{$-$} & \multicolumn{1}{c}{$-$} \\ 
$ 2.1 m_{\tau} $ & 6.604 & 6.441 & 6.685 & 3.215 & 3.449 & 6.661 \\ 
5 & 3.579 & 3.444 & 3.682 & 3.661 & 3.888 & 3.695 \\ 
10.58 & 0.7604 & 0.7073 & 0.8398 & 0.9286 & 0.9567 & 0.8373 \\ 
\hline 
\multicolumn{7}{c}{Exponentiation Type IV} \\ 
 \hline 
$ 2.1 m_{\mu} $ & 775.6 & 829.4 & 789.5 & \multicolumn{1}{c}{$-$} & \multicolumn{1}{c}{$-$} & \multicolumn{1}{c}{$-$} \\ 
0.5 & 376.7 & 393.5 & 345.7 & \multicolumn{1}{c}{$-$} & \multicolumn{1}{c}{$-$} & \multicolumn{1}{c}{$-$} \\ 
1 & 96.06 & 98.50 & 88.06 & \multicolumn{1}{c}{$-$} & \multicolumn{1}{c}{$-$} & \multicolumn{1}{c}{$-$} \\ 
2 & 24.47& 24.443& 22.58 & \multicolumn{1}{c}{$-$} & \multicolumn{1}{c}{$-$} & \multicolumn{1}{c}{$-$} \\ 
$ 2.1 m_{\tau} $ & 7.090 & 6.920 & 6.684 & 3.180 & 3.409 & 6.661 \\ 
5 & 3.870 & 3.724 & 3.682 & 3.666 & 3.888 & 3.695 \\ 
10.58 & 0.8385 & 0.7791 & 0.8397 & 0.9494 & 0.9806 & 0.8373 \\ 
%10.58 & 0.8591 & 0.7994 & 0.8413 & 0.9755 & 1.005 & 0.8414 \\
\hline 

